Spark-0: Scaling Spatially Aligned Tactile Pretraining for Robot Dexterous Manipulation

Generalist robot policies benefit from large-scale visual pretraining but often struggle with contact-rich dexterous manipulation, where force, compliance, and incipient slip are hard to observe from images. We present Spark-0, a spatially aligned vision-tactile-language-action (VTLA) model that uses touch in two complementary ways. During pretraining, image-space contact maps derived from tactile gloves, together with features from a frozen 3D geometry teacher, supervise the visual tokens; these objectives are removed at inference. In parallel, a tactile pathway encodes regional force histories and 3D taxel states to condition the action expert. A single checkpoint therefore supports both vision-only and tactile-conditioned deployment. To scale this supervision, we build HumanTouch, a 1,000-hour dataset of full-hand tactile human manipulation, and pretrain Spark-0 on it together with egocentric video, robot data, and simulation. We also release SparkArena, which pairs vision-only simulated tasks with tactile-conditioned real-robot tasks on one dexterous embodiment. Spark-0 achieves the highest mean success rate on both SparkArena tracks and ranks first on all eight aggregate metrics of the Ego Humanoid Manipulation Benchmark. Compared with vision-only pretraining on the same data and compute with touch discarded, retaining the touch of 1,000 hours of HumanTouch raises vision-only success on Ego Humanoid from 52.5% to 71.7%, and success on SparkArena-Real, where touch is also used at deployment, from 44.0% to 52.0%, indicating that touch serves not only as a policy input but also as scalable supervision for dexterous visuomotor pretraining. The Website is available at: https://xsparkai.com/Spark-0.

==> sec/6_limitations.tex <==
\section{Limitations}
\label{sec:limitations}

% 中文：本研究有五点局限。第一，人类与机器人数据共用同一种手套，向其他触觉传感器的迁移
% 尚未验证。第二，触觉条件化评测仅覆盖单一本体上的五项真机任务。第三，规模分析只有 0、100
% 和 1,000 小时触觉三个点，不足以刻画缩放规律。第四，我们未在 SparkArena-Real 上评测无触觉
% 部署，因此未单独衡量在线触觉的作用。第五，我们未单独消融几何对齐、接触对齐与触觉融合，
% 且只报告点估计，未刻画多次运行的不确定性。
Our study has five limitations. First, human and robot data share one glove
design, and transfer to other tactile sensors is untested. Second,
tactile-conditioned evaluation covers five real-robot tasks on a single
embodiment. Third, three scale anchors (0, 100, and 1,000 hours of touch)
cannot characterize a scaling law. Fourth, we do not evaluate vision-only
deployment on SparkArena-Real, so the effect of online touch alone is not
isolated. Fifth, we do not ablate geometry alignment, contact alignment, and
tactile fusion individually, and we report point estimates without
run-to-run uncertainty.


==> sec/index.tex <==
\tableofcontents
\thispagestyle{fancy}
